U-FNO -- An enhanced Fourier neural operator-based deep-learning model for multiphase flow

Numerical simulation of multiphase flow in porous media is essential for many geoscience applications. Machine learning models trained with numerical simulation data can provide a faster alternative to traditional simulators. Here we present U-FNO, a novel neural network architecture for solving multiphase flow problems with superior accuracy, speed, and data efficiency. U-FNO is designed based on the newly proposed Fourier neural operator (FNO), which has shown excellent performance in single-phase flows. We extend the FNO-based architecture to a highly complex CO2-water multiphase problem with wide ranges of permeability and porosity heterogeneity, anisotropy, reservoir conditions, injection configurations, flow rates, and multiphase flow properties. The U-FNO architecture is more accurate in gas saturation and pressure buildup predictions than the original FNO and a state-of-the-art convolutional neural network (CNN) benchmark. Meanwhile, it has superior data utilization efficiency, requiring only a third of the training data to achieve the equivalent accuracy as CNN. U-FNO provides superior performance in highly heterogeneous geological formations and critically important applications such as gas saturation and pressure buildup "fronts" determination. The trained model can serve as a general-purpose alternative to routine numerical simulations of 2D-radial CO2 injection problems with significant speed-ups than traditional simulators.

==> r2table.tex <==

\begin{table}[h]
\scriptsize
    \centering
    \caption{Average training and testing data set R$^2$ scores of 500 random samples for 4 models. $R^2$ scores measures the similarity between the prediction and the numerical simulation output; an $R^2$ of 1 indicates an exact match. }
    \begin{tabular}{c|cc|cc|cc|cc}
              \hline
        \multirow{3}{*}{Model} & \multicolumn{4}{c|}{Gas saturation ($SG$)} & \multicolumn{4}{c}{Pressure buildup ($dP$)} \\
        \cline{2-9}
        & \multicolumn{2}{c|}{Train} & \multicolumn{2}{c|}{Test}& \multicolumn{2}{c|}{Train } & \multicolumn{2}{c}{Test }\\
        & mean &  std &  mean & std & mean &  std &  mean & std \\
              \hline
        CNN &  0.994 & 0.007 & 0.986 & 0.018 & 0.990 & 0.029 & 0.988 & 0.023 \\
        FNO &  0.990 & 0.013 & 0.986 & 0.017 & 0.991 & 0.014 & 0.990 & 0.017 \\
        Conv-FNO & 0.993 & 0.011 & 0.990 & 0.013 & 0.992  &  0.018 & 0.991 & 0.018  \\
        \textbf{U-FNO} &  \textbf{0.997} & \textbf{0.005} & \textbf{0.994} & \textbf{0.009} & & &  & \\
              \hline
    \end{tabular}
    \label{tab:r2}
\end{table}
